HADAS Green Assistant: designing energy-efficient applications

The number of works addressing the role of energy efficiency in the software development has been increasing recently. But, designers and programmers still complain about the lack of tools that help them to make energy-efficiency decisions. Some works show that energy-aware design decisions tend to have a larger impact in the power consumed by applications, than code optimizations. In this paper we present the HADAS green assistant, which helps developers to identify the energy-consuming concerns of their applications (i.e., points in the application that consume more energy, like storing or transferring data), and also to model, analyse and reason about different architectural solutions for each of these concerns. This tool models the variability of more or less green architectural practices and the dependencies between different energy-consuming concerns using variabilty models. Finally, this tool will automatically generate the architectural configuration derived from the selections made by the developer from an energy consumption point of view.

==> assistent.tex <==
\section{Green Assistant Overview}
In this section we will give an overview of the HADAS Green Assistant tool, from the user point of view. So, we will show first how to use it, before presenting the complexity of implementing such a tool.
Suppose Alice is a software developer that wants to develop an energy-efficient application. If she wants to use the HADAS Green assistant, she must follow the following steps also shown in Figure \ref{fig:assistant}:



%\begin{figure}[!t]
%    \begin{center}
%        \includegraphics[scale=0.41]{/Figures/Assistant}
%    \end{center}   
%    \caption{Green Assistant Overview.}
%    \label{fig:assistant}
%\end{figure}


\begin{enumerate}
\item Identify energy hotspots in the application requirements. Alice wants to develop a photo gallery application, so she needs to add a photo in an album and to reduce the photo quality of a photo, among other functionality. The HADAS green assistant has previously identified these concerns as energy consuming. For instance, data store (e.g., add a photo) and file compression (e.g., reduce the quality of a photo). 
\item Select the energy-consuming concerns in the Hadas Repository. Alice can see the data store and the file compression in the repository of energy consuming concerns showed by the HADAS green assistant. She should select all the energy-consuming concerns provided by HADAS that she needs to develop the application. Now Alice knows that these concerns may strongly affect the final energy expenditure of her application. The user interface is implemented as a Google Form, that fits very well what we need. This Google Form (see Figure X) has a extensive list with all the concerns (e.g., Store, Communication, Compression or Security) and although they are pretty intuitive, in the form we also show some keywords that could could be associated with each of these concerns. For example, the Store concern could be used when in the application requirements the developer finds words like, save, upload, add, send, put, write, among others.
\item Choose the options for every energy-consuming concern selected in Step 2. HADAS will show the application developer a separated form for every selected concern and in our case Alice has to select the alternatives she wants to use. For instance, the photo storing could be done in locally and/or remotely in an external hard drive and or in the cloud. Depending on this selection, alternatives for other energy consuming concerns could be also suggested by the assistant. For example if the developer choose the cloud remote storage option this implies that the photos have to be uploaded to a remote server. But, the Communication concern that is the responsible for sending the file to the cloud, was previously identified by HADAS as another energy consuming concern. Then, in order to make easier the developer job, HADAS automatically will show a list with the different alternatives of the Communication concern, so as Alice can choose one of them. If Alice chooses the external hard drive as remote storage, this solution could need encryption, that is another energy consuming concern according to HADAS. So, alternatives security-related concerns will also be shown to the developer.
\item Energy-efficiency Analysis of the different alternatives explored by the developer. After Alice selected the architectural solution she wants for every energy consuming concern in step 3), HADAS will help her to be aware of the energy implications of their decisions. The energy consumption of each alternative is expressed by means of energy functions parameterized by variable parameters (e.g., the photo file size). HADAS does not provide the exact consumption in Watts, but what Alice needs to know is which alternatives are more energy consuming than others and which ones can be considered more green. This is an iterative process, since Alice can select different options and analyse the impact of each of her decisions in the energy expenditure of the application. Thanks that HADAS take into account the dependencies between different energy consuming concerns, Alice will be able to take complex decisions about no so much effort. For example, Alice can decide not to include the possibility of cloud remote storage for uncompressed files. She was able to make this decision, because the expected size of photos is large enough to justify including extra components for compressing and uncompressing the file.%%LIDIA: esto ultimo era mas o menos lo que ponia pero no se si es cierto, habria que verlo
HADAS cannot decide on behalf of Alice, unless she decided not to select any option of some of the energy consuming concerns. %%LIDIA: no se si somos capaces de decidir por defecto un determinada opcion, y generar aquella solucion que consume menos energia segun algun parametro o considerando el tamaño mas pequeño
\item Get the architectural configuration and add other functionality. Finally, HADAS will provide the architectural configuration including the definitive options the developer selected after the analysis of the step 4). For instance, HADAS will provide the configuration of the Store, Compression, Security and Comunnication concerns with the option choosen by the developer. In this case Alice, will have to complete the application with the rest of the functionality considered not relevant for energy efficiency (e.g., photo edition)
\end{enumerate}

